A Resourceful Coordination Approach for Multilevel Scheduling

HPC users aim to improve their execution times without particular regard for increasing system utilization. On the contrary, HPC operators favor increasing the number of executed applications per time unit and increasing system utilization. This difference in the preferences promotes the following operational model. Applications execute on exclusively-allocated computing resources for a specific time and applications are assumed to utilize the allocated resources efficiently. In many cases, this operational model is inefficient, i.e., applications may not fully utilize their allocated resources. This inefficiency results in increasing application execution time and decreasing system utilization. In this work, we propose a resourceful coordination approach (RCA) that enables the cooperation between, currently independent, batch- and application-level schedulers. RCA enables application schedulers to share their allocated but idle computing resources with other applications through the batch system. The effective system performance (ESP) benchmark is used to assess the proposed approach. The results show that RCA increased system utilization up to 12.6% and decreased system makespan by the same percent without affecting applications' performance.

==> background.tex <==
\section{Background}
\label{sec:background}
%This section mainly spans two research areas: batch and application scheduling, with, highlights of the most common scheduling techniques \ahm{in each area}.  
%The scheduling libraries and the runtime systems that employ such application and batch scheduling techniques are \ahm{also} discussed.
%\ahm{T}his section also reviews specific \ahm{notable} scheduling simulators and simulation frameworks that were used in the literature to study application and batch level scheduling techniques.
\textbf{\ahm{Batch-level} scheduling (BLS) and resource and job management systems:}
A batch system, also known as a RJMS, is the middleware responsible for resource allocation (RA) and for managing job execution on the allocated resources~\cite{georgiou2012evaluating}. 
One can consider the RJMS to be the operating system of an HPC system.

A RJMS has four main responsibilities~\cite{reuther2018scalable}:~(1) managing job life cycle from submission to execution, including placing jobs into queues and prioritizing them, (2)~tracking resources' usage and availability, (3)~allocating resources to jobs (batch scheduling), and (4)~dispatching and launching jobs on the allocated resources.
%PBS~\cite{henderson1995job}, Grid Engine~\cite{GridEngine}, IBM LSF, and Slurm~\cite{yoo2003slurm} are examples of \mbox{well-known} and commonly used RJM systems.
RJMS employ various batch scheduling techniques: the \emph{\mbox{first-come-first-serve}}~(FCFS) technique, which assigns the highest priority to the job with the earliest arrival time; 
the \emph{earliest deadline first}~(EDF) technique, which assigns the highest priority to the job with the earliest deadline;
and the \emph{shortest job first}~(SJF) technique, which assigns the highest priority to the job with the shortest execution time~\cite{azmi2011scheduling}.
Most RMJS exhibit \mbox{user-defined} scheduling techniques by offering a generic way to prioritize jobs based on various factors, including fairness~\cite{hovestadt2003scheduling}, quality of service criteria, and others. 
However, in practice, HPC administrators usually employ a simple configuration of FCFS with backfilling~(BF).
Backfilling~\cite{BF} is a supporting scheduling technique that helps to increase system utilization by executing small jobs (which request a small number of computing resources) when there are insufficient available computing resources to assign to the highest priority jobs.

\textbf{BLS  simulation:}
%Batch scheduling is among the responsibilities of a \ahm{RMJS}. 
%\ahm{RMJS} consist of several interacting components.
The performance of a batch scheduling policy is affected by the overhead of other RMJS components.
For instance, dispatching and launching jobs on the allocated resources require executing epilog and prolog scripts on the allocated resource, which incurs overhead.

Capturing the mutual effect between the various RMJS components is a challenging task.
%Batch simulators can be either based on \mbox{real-life} RJM systems or based on simulation frameworks~\cite{klusavcek2019alea}.
Therefore, certain batch simulators are based on the actual source code of production RJMS.
For instance, the Slurm simulator~\cite{lucero2011simulation} is based on the Slurm RJMS~\cite{yoo2003slurm}. %, while Simbatch and Alea~\cite{klusavcek2010alea,klusavcek2007alea} are based on SimGrid~\cite{SimGrid} and GridSim~\cite{GridSim}, respectively.
%Each types of these simulations has its advantages and disadvantages.
%For instance in \mbox{real-life}  RJM based simulation, a batch scheduled is not an isolated component.
Hence, the \mbox{Slurm-based} simulation captures the effects of various RJMS components on the scheduling.
Most \mbox{open-source} RJMS are written using a complex and large code base that is often insufficiently documented.
Consequently, adding new or extending existing scheduling techniques in \mbox{RJMS-based} simulators inherits this complexity.
In the present work, we implemented our proposed approach in a \mbox{Slurm-based} simulator~\cite{simakov2017slurm}.
\out{This introduced the challenge of understanding the source code of the actual Slurm RJMS. 
However, this knowledge will facilitate the future integration of the proposed approach into the production Slurm RJMS.}

\textbf{\ahm{Application-level} scheduling~(ALS):}
%Most of scientific applications are iterative applications by nature~\cite{furlinger2010recording}, such as \mbox{time-stepping} applications~\cite{fractiling}, and linear solvers~\cite{golub1997closer}.
%The iterative nature is reflected in applications' code as large loops (hundred thousands and millions of iterations ).
Loops are  the prime source of parallelism in scientific applications~\cite{fang1990dynamic}.
Efficient scheduling of loop iterations enhances applications' performance, and therefore, one may consider loop scheduling as an excellent representative of \mbox{application-level} scheduling~(ALS). 
On \mbox{large-scale} HPC systems, efficient loop execution is challenging, because the latest finishing computing resource dictates the entire parallel loop execution time.
Many factors cause imbalanced executions of loop iterations, including \textit{problem}, \textit{algorithmic}, and \textit{systemic} characteristics.
\ahm{For instance,  heterogeneous processors of computing systems, nonuniform memory access (NUMA) effect,  and operating system noise cause load imbalance.}
Loop scheduling aims to balance loop iterations' execution across available computing resources and over  time.
%Loop scheduling techniques can be categorized as static or dynamic  techniques.
%Static loop scheduling~(SLS) divides and assigns loop iterations before application execution~\cite{lilja1994exploiting,li1993locality}.
%Dynamic loop scheduling~(DLS) divides and assigns loop iterations during application execution.
%Furthermore,  DLS techniques can be either nonadaptive or adaptive.
%The major difference between nonadaptive and adative DLS is adaptive techniques revise their scheduling decisions based on profiling information obtained during application execution. 
%that represent the aforementioned loop scheduling categories 
In the current work, three scheduling techniques were selected: static~(STATIC)~\cite{li1993locality}, guided self-scheduling~(GSS)~\cite{GSS}, and adaptive factoring~(AF)~\cite{AF}.
STATIC~\cite{li1993locality} is a straightforward parallelization. 
It assigns each computing resource  a chunk of loop iterations that is equal to $\ceil{N/P}$, where $N$ and $P$ are the total number of loop iterations and the total number of computing resources, respectively.
GSS is a dynamic \mbox{self-scheduling} technique that uses a \mbox{non-linear} function to self-schedule a decreasing chunk sizes.
At every scheduling step, GSS divides the remaining loop iterations by the total number of processing elements.
%FAC is a dynamic \ahm{\mbox{self-scheduling}} technique that evolves from comprehensive probabilistic analyses.
%It \ahm{divides and self-schedules} loop iterations in batches of \mbox{equal-sized} chunks \ahm{to the free and requesting computing resources}.
%To calculate the optimal batch size, FAC requires prior knowledge of the mean $\mu$ and the standard deviation $\sigma$ of the loop iterations execution times.
AF~\cite{AF} is an adaptive \mbox{self-scheduling} technique that is based on the factoring~(FAC) technique~\cite{FAC}.
FAC requires prior knowledge of the mean $\mu$ and the standard deviation $\sigma$ of the loop iterations execution times.
Unlike FAC, AF learns both $\mu$ and $\sigma$ for each computing resource during applications' execution to ensure full adaptivity to all factors that cause load imbalance.

%\subsection{DLS Libraries at ALS}
%\label{sec:background_lb_via_dls}
%DLS techniques have been used to balance loop execution across several computing resource.
%For both \mbox{shared-memory} and \mbox{distributed-memory} systems, DLS technique have shown performance advantages in several scientific applications~\cite{fractiling,golub1997closer,kasielke2019exploring,Eleliemy:hpcc,psia}.
%The OpenMP standard offers three alternatives that a developer can use to balance the execution of any given loop.
%These three options are static, dynamic, and guided.  
%\textit{Static} is equivalent to the block cyclic~\cite{li1993locality} technique where chunks of loop iterations (block) are distributed in a round-robin fashion (cyclic).
%For static, the default chunk size is $\ceil{N/P}$, where $N$ and $P$ are the total number of loop iterations and the total number of computing resources, respectively.
%\textit{Dynamic} assigns chunks in a dynamic order that is defined during execution, i.e., once a thread is free and available, it obtains a new chunk.
%When the chunk size of dynamic equals one loop iterations, dynamic is equivalent to the \mbox{self-scheduling}~(SS)~\cite{SS} technique.
%\textit{Guided} follows the same execution scheme of dynamic; once a thread is free and available it obtains a new chunk. 
%However, guided assigns chunks of \textit{decreasing} sizes.
%The chunk size of guided equals  $\ceil{R/P}$, where $R$ and $P$ are the current remaining loop iterations and the total number of computing resources, respectively.
%The guided scheduling option in OpenMP is equivalent to the guided \mbox{self-scheduling}~(GSS)~\cite{GSS}. 
%%Table~\ref{tab:mapping} summaries the OpenMP options and their corresponding techniques.
%The OpenMP standard also has an option to determine the selected loop scheduling techniques during applications' execution.
%Recent research efforts extensively extended the OpenMP runtime libraries to add more DLS techniques.
%For instance, a research effort~\cite{Ciorba:2018} extended the GNU \mbox{LaPeSD-libGOMP}~\footnote{https://github.com/lapesd/libgomp} runtime library by adding four DLS techniques, including trapezoid \mbox{self-scheduling} (TSS)~\cite{TSS}, FAC~\cite{FAC}, weighted factoring~(WF)~\cite{WF} and random~\cite{Ciorba:2018}.
%Another research effort~\cite{korndorferruntime} extended the LLVM implementation of the OpenMP runtime library with eleven DLS techniques, including fixed size chunk~(FSC)~\cite{FSC}, FAC~\cite{FAC}, Taper (TAP)~\cite{TAP}, weighted factoring~(WF)~\cite{WF}, bold~(BOLD)~\cite{BOLD}, adaptive weighted factoring and its variants \mbox{AWF-B}, \mbox{AWF-C}, \mbox{AWF-D}, and \mbox{AWF-E}~\cite{AWF,AWFBC}, and adaptive factoring~(AF)~\cite{AF}. 
%\begin{table}[!h]
%	\centering
%	\caption{Mapping between OpenMP schedule clause options and DLS techniques}
%	\label{tab:mapping}
%	\begin{tabular}{l|l}
%		DLS technique & OpenMP schedule clause \\ \hline
%		schedule(static)   & STATIC~\cite{li1993locality}           \\
%		schedule(dynamic,1)  & SS~\cite{SS}             \\
%		schedule(guided,1)  & GSS~\cite{GSS}           
%	\end{tabular}
%\end{table}

%the MPI standard offers several functions that a developer uses to handle message exchanges between MPI processes. 
%However
%For \mbox{distributed-memory} systems, the MPI standard lacks support for scheduling functions that can be used to distribute and schedule execution of loop iterations.

%Several research efforts introduced and developed \mbox{MPI-based} libraries to support loop scheduling~\cite{LBtool,DLBLtool,processorgroups,mohammed2019approach}.
%A \mbox{load-balancing} tool, called~\mbox{DLB\_tool}~\cite{LBtool} employed several DLS techniques.
%The \mbox{DLB\_tool} exploited a \mbox{master-worker}, where a single computing resource, called master, is responsible for chunk calculation and assignment. 
%In the \mbox{DLB\_tool}, the master also executes chunks of loop iteration as a normal worker.

%An enhanced tool for dynamic load balancing, called  dynamic load balancing library~(DLBL)~\cite{DLBLtool} included the same set of DLS techniques of the \mbox{DLB\_tool}.
%The DLBL was the first to utilize MPI \mbox{one-sided} communication, where the master process receives work requests, and for each request, it calculates the size of the new chunk.
%The master process calls a handler function on the worker side. 
%Workers obtain the data of the new chunks from the master process without any further involvement from the master.

%Another research effort~\cite{processorgroups} proposed a new execution model implement DLS techniques. 
%This new execution model divides the computing resources into groups.
%Each group is responsible for scheduling of a specified portion of the iteration space.
%Each group implements a DLS technique using a traditional \mbox{master-worker} model.
%However, the master of each group periodically reports the ratio of the remaining iterations and the available workers to a global master, called manager. 
%When the reported ratio exceeds a certain threshold, the manager migrates workers between processor groups.

%Recently, an extended version of the \mbox{DLB\_tool}, called DLS4LB, was introduced~\cite{mohammed2019simas}.
%The DLS4LB added four DLS techniques to the DLB tool.
%The DLS4LB  also advanced the DLB tool by adding a \mbox{simulator-assisted} (SimAS) scheduling approach that dynamically selects the best DLS technique during execution. 
%SimAS exploits application characteristics and the present state of the
%computing system to predict application behavior when employing a particular DLS technique, and consequently, it selects the techniques with the best predicted performance. 
%A common aspect of all these libraries is that they exploit a \mbox{master-worker} model and assume replicated data among all computing resources.

\textbf{ALS simulation:}
%Various DLS techniques have been extensively studied via simulation~\cite{AhmedSC16,srivastava2011enhancing,Ali_HPCC:17,dlsmsg,hoffeins2017examining,Mohammed:2018a} \ahm{in} two main simulation frameworks: SimGrid~\cite{SimGrid} and GridSim~\cite{GridSim}.
Various dynamic loop scheduling~(DLS) techniques have extensively been studied via simulation~\cite{AhmedSC16,srivastava2011enhancing,Mohammed:2018a} in two main simulation frameworks: SimGrid~\cite{SimGrid} and GridSim~\cite{GridSim}.
Eight DLS techniques were implemented~\cite{mahad} using one SimGrid interface, called MSG, i.e., the authors evaluated the scalability of these DLS techniques in the presence of algorithmic and systemic variations.
The SimGrid simulator was used to verify the implementation of DLS techniques~\cite{Mohammed:2018a}.
Alea~\cite{klusavcek2010alea,klusavcek2007alea} is an \mbox{event-based} simulator that is based on GridSim~\cite{GridSim}. 
Alea was extended to support four DLS techniques~\cite{srivastava2011enhancing}.

Both SimGrid and Alea were used to simulate DLS techniques.
However, SimGrid outperforms Alea with regards to simulator \mbox{wall-clock} time~\cite{AhmedSC16}.
For this reason, in the present work, we use and extend the latest verified \mbox{SimGrid-based} simulator~\cite{mohammed2019approach} to simulate the execution of scientific applications with various DLS techniques on HPC systems.


%Alea~\cite{klusavcek2010alea,klusavcek2007alea} is a \mbox{GridSim-based} simulator simplified the DLS development and brought unique advantages to DLS simulation, including reading job files written in standard workload format (SWF) \cite{swfchapin1999benchmarks}.
 

 
%5Since scheduling is a very hard problem and implementing a scheduling software for HPC production systems involves numerous technical details, simulation approaches have been widely used to examine performance of different scheduling algorithms. 
%Two simulation toolkits, GridSim~\cite{GridSim} and SimGrid~\cite{SimGrid} have been used to develop DLS techniques in simulation. 

%GridSim facilitates simulation of grids, clusters, and single processing elements. 
%In fact, it supports a range of heterogeneous resources including shared and distributed memory architectures.
%Alea~\cite{,} is \mbox{well-known} simulator that employs the GridSim toolkit.
%Alea exhibits several advantage, including (1) Reading jobs files written in standard workload format (SWF) \cite{swfchapin1999benchmarks} and (2) Reading of platform files instead of defining the simulated platform within the code. 
%Moreover, Alea has a central scheduler module responsible for applying different scheduling algorithms and allocation policies.
%Therefore, several research efforts used Alea to simulate DLS techniques~\cite{AhmedSC16}.
%For instance,  Srivastava et. al. extended Alea to support four DLS techniques, including  SS, FSC, GSS,and  FAC~\cite{srivastava2011enhancing}.
%Using Alea, the authors studied and assessed the scalability of these techniques in several scenarios.


%SimGrid~\cite{SimGrid}  is another remarkable simulation toolkit. 
%Unlike GridSim that focuses on simulating scheduling algorithms and resource allocation policies at grid and cluster levels, SimGrid supports the simulation of parallel and distributed applications in heterogeneous/homogeneous parallel and distributed environments.
%SimGrid offers three interfaces to develop different simulations: SimDag, MSG, and SMPI.
%The three interfaces were used in various research efforts to simulate DLS techniques.
%For instance using MSG, eight DLS techniques, including  SS~\cite{SS}, FSC~\cite{FSC}, GSS~\cite{GSS}, FAC~\cite{FAC}, WF~\cite{WF}, \mbox{AWF-B}, \mbox{AWF-C}~\cite{AWFBC}, and AF~\cite{AF} were implemented~\cite{mahad}.
%The authors evaluated the scalability of these DLS techniques  in the presence of algorithmic and systemic variations.
%Furthermore, both of the MSG and SimDag interface were used to verify the implementation of DLS techniques~\cite{Ali_HPCC:17,dlsmsg,hoffeins2017examining,Mohammed:2018a}


